Rieoptax: Riemannian Optimization in JAX

We present Rieoptax, an open source Python library for Riemannian optimization in JAX. We show that many differential geometric primitives, such as Riemannian exponential and logarithm maps, are usually faster in Rieoptax than existing frameworks in Python, both on CPU and GPU. We support various range of basic and advanced stochastic optimization solvers like Riemannian stochastic gradient, stochastic variance reduction, and adaptive gradient methods. A distinguishing feature of the proposed toolbox is that we also support differentially private optimization on Riemannian manifolds.

==> abstract.tex <==
\begin{abstract}%
    We present Rieoptax, an open source Python library for Riemannian optimization in JAX. We show that many differential geometric primitives, such as Riemannian exponential and logarithm maps, are usually faster in Rieoptax than existing frameworks in Python, both on CPU and GPU. We support various range of basic and advanced stochastic optimization solvers like Riemannian stochastic gradient, stochastic variance reduction, and adaptive gradient methods. A distinguishing feature of the proposed toolbox is that we also support differentially private optimization on Riemannian manifolds. 
\end{abstract}

==> manuscript.tex <==

\section{Introduction}
Riemannian geometry is a generalization of the Euclidean geometry \cite{lee2006riemannian, helgason1979differential} to general Riemannian manifolds. It includes several nonlinear spaces such as the set of positive definite matrices \cite{bhatia2009positive,thanwerdas2021n}, Grassmann manifold of subspaces~\cite{edelman1998geometry,bendokat2020grassmann, absil2009optimization}, Stiefel manifold of orthogonal matrices~\cite{edelman1998geometry,absil2009optimization, chakraborty2019statistics},  Kendall shape spaces \cite{kendall1984shape,kendall1989survey, miolane2017template}, hyperbolic spaces \cite{ungar2008gyrovector, ungar2008analytic}, and special Euclidean and orthogonal group \cite{selig2005geometric, gallier2020differential, sola2018micro}, to name a few. 


Optimization with manifold based constraints has become increasingly popular and has been employed in various applications such as low rank matrix completion~\cite{boumal2011rtrmc}, learning taxonomy embeddings~\cite{nickel2017poincare,nickel2018learning},  neural networks~\cite{huang2017riemannian, huang2017deep, huang2018building, ganea2018hyperbolic, nguyen2019neural,qi2021transductive}, density estimation \cite{hosseini2020alternative, han2021riemannian}, optimal transport \cite{chewi2020gradient,altschuler2021averaging, shi2021coupling,mishra2021manifold,han2022riemannianblockSPD}, shape analysis~\cite{srivastava2010shape,  huang2016riemannian}, and topological dimension reduction~\cite{kachan2020persistent}, among others. 
% However, current libraries for Riemannian optimization are not efficient, particularly for large-scale and high-dimensional applications \PJcomment{this statement is a bit strong and general - can we say some specific aspect of efficiency that they lack? Like GPU support? e.g., from what I remember, Manopt and Pymanopt does not have GPU implementation}. 


In addition, privacy preserving machine learning \cite{dwork2006calibrating,dwork2006our,dwork2008differential,chaudhuri2011differentially,song2013stochastic, abadi2016deep, mironov2017renyi} has become crucial in real applications, which has been generalized to manifold-constrained problems very recently \cite{reimherr2021differential,utpala2022differentially,han2022differentially}. Nevertheless, such a feature is absent in existing Riemannian optimization libraries \cite{boumal2014manopt,bergmann2022manopt,meghwanshi2018mctorch,kochurov2020geoopt,smirnov2021tensorflow,JMLR:v17:16-177,miolane2020geomstats}. 

In this work, we introduce Rieoptax (\textbf{Rie}mannian \textbf{Opt}imization in J\textbf{ax}), an open source Python library for Riemannian optimization in JAX \cite{frostig2018compiling, jax2018github}. 
The proposed library is mainly driven by the needs of efficient implementation of manifold-valued operations and optimization solvers, readily compatible with GPU and even TPU processors as well as the needs of privacy-supported Riemannian optimization. To the best of our knowledge, Rieoptax is the first library to provide privacy guarantees within the Riemannian optimization framework. 
% To this end, we propose Rieoptax, which is a python library based on JAX \cite{frostig2018compiling, jax2018github}. 



\subsection{Background on Riemannian optimization, privacy, and JAX}


\paragraph{Riemannian optimization.}
Riemannian optimization \cite{absil2009optimization, boumal2022intromanifolds} considers the following problem
\begin{align}
    \min_{w \in \mathcal{M}} f(w), \label{Eq:OPT}
\end{align}
where $f : \mathcal{M} \rightarrow \mathbb{R}$, and $\mathcal{M}$ denotes a Riemannian manifold. 
%Applications of \eqref{Eq:OPT} are pervasive in machine learning. 
%Some of the most popular examples are low rank matrix completion \cite{boumal2011rtrmc}, learning taxonomy embeddings \cite{nickel2017poincare,nickel2018learning},  training neural networks with manifold constraints \cite{huang2017riemannian, huang2017deep, huang2018building,nguyen2019neural,qi2021transductive}, optimal transport \cite{chewi2020gradient,altschuler2021averaging, shi2021coupling,mishra2021manifold,han2022riemannianblockSPD}, shape analysis \cite{srivastava2010shape,  huang2016riemannian}, topological dimension reduction \cite{kachan2020persistent}, among others. 
Instead of considering \eqref{Eq:OPT} as a constrained problem, Riemannian optimization \cite{absil2009optimization, boumal2022intromanifolds} views it as an unconstrained problem on the manifold space. Riemannian (stochastic) gradient descent \cite{zhang2016first,bonnabel2013stochastic} generalizes the Euclidean gradient descent with intrinsic updates on manifold, i.e., $w_{t+1} = {\rm Exp}_{w_t}(- \eta_t \, {\rm grad} f(w_t))$, where ${\rm grad} f(w_t)$ is the Riemannian (stochastic) gradient, ${\rm Exp}_w(\cdot)$ is the Riemannian exponential map at $w$ and $\eta_t$ is the step size. 
% Several kinds of algorithms have been developed to solve \eqref{Eq:OPT}. Riemannian (stochastic) gradient descent \cite{zhang2016first,bonnabel2013stochastic},
Recent years have witnessed significant advancements for Riemannian optimization where more advanced solvers are generalized from the Euclidean space to Riemannian manifolds. These include
variance reduction methods \cite{zhang2016riemannian, sato2019riemannian, kasai2018riemannian, zhou2019faster, hanmomentum2021,han2021improved}, adaptive gradient methods \cite{becigneul2018riemannian, kasai2019riemannian}, accelerated gradient methods \cite{han2022riemannian, liu2017accelerated,ahn2020nesterov,zhang2018estimate, alimisis2020continuous}, quasi-Newton methods \cite{huang2015broyden,qi2010riemannian}, zeroth-order methods \cite{li2022stochastic} and second order methods, such as trust region methods \cite{absil2007trust} and cubic regularized Newton's methods \cite{agarwal2021adaptive}. 


\paragraph{Differential privacy on Riemannian manifolds.}  Differential privacy ({DP}) provides a rigorous treatment for data privacy by precisely quantifying the deviation in the model's output distribution under modification of a small number of data points \cite{dwork2006calibrating,dwork2006our,dwork2008differential,dwork2014algorithmic}. Provable guarantees of {DP} coupled with properties like immunity to arbitrary post-processing and graceful composability have made it a de-facto standard of privacy with steadfast adoption in the real applications \cite{erlingsson2014rappor, apple2017learning,ding2017collecting, near2018differential, abowd2018us}. Further, it has been shown empirically that {DP} models resist various kinds of leakage attacks that can cause privacy violations \cite{rahman2018membership, 10.5555/3361338.3361358,sablayrolles2019white,zhu2019deep,balle2022reconstructing}.



Recently, there is a surge of interest on differential privacy over Riemannian manifolds, which has been explored in the context of Fr\'echet mean~\cite{frechet1948elements} computation~\cite{reimherr2021differential,utpala2022differentially} and, more generally, empirical risk minimization problems where the parameters are constrained to lie on a Riemannian manifold~\cite{han2022differentially}. 




\paragraph{JAX and its ecosystem.} JAX \cite{frostig2018compiling, jax2018github} is recently introduced machine learning framework which support automatic differentiation capabilities \cite{baydin2018automatic} via  \texttt{grad()}. Further some of the distinguishing features of JAX are just-in-time (JIT) compilation using the accelerated linear algebra (XLA) compiler \cite{50530} via \texttt{jit()}, automatic vectorization (batch-level parallelism) support with \texttt{vmap()}, and strong support for parallel computation via \texttt{pmap()}.  All the above transformations can be composed arbitrarily because JAX follows the functional programming paradigm and implements these as pure functions. 



% JAX also enables vectorizing maps (functions), known as \texttt{vmap}, that allows efficient batch level parallelism. 
%Additionally, one of core functions present in JAX is \texttt{vmap}, a vectorized map, which enables easy-to-write and efficient batch level parallelism. 

Given that JAX has many interesting features, its ecosystem has been constantly expanding in the last couple of years. Examples include neural network modules (Flax \cite{flax2020github}, Haiku \cite{haiku2020github}, Equinox \cite{kidger2021equinox}, Jraph \cite{jraph2020github}, Equivariant-MLP \cite{finzi2021practical}), reinforcement learning agents (Rlax \cite{deepmind2020jax}), Euclidean optimization algorithms (Optax \cite{deepmind2020jax}), federated learning (Fedjax \cite{fedjax2021}), optimal transport toolboxes (Ott \cite{cuturi2022optimal}), sampling algorithms (Blackjax \cite{blackjax2020github}), differential equation solvers (Diffrax \cite{kidger2021on}), rigid body simulators (Brax \cite{brax2021github}), and differentiable physics (Jax-md \cite{jaxmd2020}), among others. 

% \begin{center}
%     \textit{However, support for Riemannian optimization in JAX is missing.} \AHcomment{(to be removed?)}
% \end{center} 

\subsection{Rieoptax} 

We believe that the proposed framework for Riemannian optimization in JAX is a timely contribution that brings several benefits of JAX and new features (such as privacy support) to the manifold optimization community discussed below.
% \PJcomment{does this look ok?}

\begin{itemize}
    \item \textbf{Automatic and efficient vectorization with} \texttt{vmap().} Functions that are written for inputs of size $1$ can be converted to functions that take batch of inputs by wrapping it with \texttt{vmap()}. For example, the function \texttt{def dist(point\_a, point\_b)} for computing distance between a single \texttt{point\_a} and a single \texttt{point\_b} can be converted to function that computes distance between a batch of \texttt{point\_a} and/or a batch \texttt{point\_b} by wrapping \texttt{dist} with \texttt{vmap()} without modifying the \texttt{dist()} function. This is useful in many cases, e.g., Fr\'echet mean computation $\min_{w \in \mathcal{M}} \left\{ \frac{1}{n} \sum_{i=1}^{n} f_{i}(w) := \frac{1}{n} \sum_{i=1}^{n} \text{dist}^2(w,z_i)\right\}$. Furthermore, vectorization with \texttt{vmap()} is usually faster or on par with manual vectorization \cite{jax2018github}. 
    % Example: consider Frechet mean \cite{frechet1948elements} as follows,  
    % \begin{align*}
    %     \min_{w \in \mathcal{M}} \left\{ \frac{1}{n} \sum_{i=1}^{n} f_{i}(w) \delequal \frac{1}{n} \sum_{i=1}^{n} \text{dist}^2(w,z_i)\right\}.
    % \end{align*}
    \item \textbf{Per-example gradient clipping.} A key process in differentially private optimization is per-example gradient clipping $ \frac{1}{n}\sum_{i=1}^{n} \text{clip}_{\tau}(\text{grad} f_{i}(w))$ , where $\text{clip}_{\tau}$ ensures norm is atmost $\tau$.  
    % \begin{align*}
    %    \frac{1}{n}\sum_{i=1}^{n} \text{clip}_{\tau}(\text{grad} f_{i}(w)).  
    % \end{align*}
    Here, the order of operations is important: the gradients are first clipped and then averaged. Popular libraries including Autograd~\cite{maclaurin2015autograd}, Pytorch~\cite{paszke2019pytorch} and Tensorflow~\cite{abadi2016tensorflow} are heavily optimized to directly compute the mean gradient $\frac{1}{n}\sum_{i=1}^{n} \text{grad} f_{i}(w)$ and hence do not expose per-example gradients i.e., $\text{grad} f_{i}(w).$ Hence, one has to resort to ad-hoc techniques \cite{goodfellow2015efficient,  rochette2019efficient, lee2021scaling} or come up with algorithmic modifications \cite{bu2021fast} which inherently have speed versus performance trade-off. JAX, however, offers native support for handling such scenarios and JAX-based differentially private Euclidean optimization methods have been shown to be much faster than their non-JAX counterparts~\cite{subramani2021enabling}. We observe that JAX offer similar benefits for differentially private Riemannian optimization as well. 
    %has been shown to be couple of orders magnitude faster \cite{subramani2021enabling}. Although all these observations have been made  in context of deferentially private Euclidean optimization, these hold for  differentially private Riemannian optimization as well. 
    
     \item \textbf{Single Source Multiple Devices (SSMD) paradigm.} JAX follows the SSMD paradigm, and hence, the code written for CPUs can be run on GPU/TPUs without any additional modification.
     
    %  \PJcomment{This is advantageous particularly becasue the popular Riemannian optimization libraries like Pymanopt~\citep{JMLR:v17:16-177} have only CPU-based implementation and currently require significant effort if they wish to offer GPU and TPU support.} \STcomment{Geoopt, Tf-Riemnopt offer GPU support}
\end{itemize}




Rieoptax is available at \url{https://github.com/SaitejaUtpala/Rieoptax/}.




% \PJcomment{yes, link will be great}
% \AHcomment{(Shall we put up a github link? But I think it needs to be anonymous.)}
% \STcomment{(I have contacted organizers. there provided a way to make it anonymous)}
% \AHcomment{(Okay)} 

\section{Design and Implementation overview}

The package currently implements several commonly used geometries, optimization algorithms and differentially private mechanisms on manifolds. More geometries and advanced solvers will be added in the future.



\subsection{Core}

\begin{itemize}
    \item \texttt{rieoptax.core.ManifoldArray:} lightweight wrapper of the \texttt{jax} device array with \texttt{manifold} attribute and used to model array constrained to manifold. It is registered as \texttt{Pytree} to ensure compatibility jax primitives like \texttt{grad()} and \texttt{vmap()}. 
    
    % \item \texttt{rieoptax.core.TangentArray:} Used to model tangent vector contains value (\texttt{jax} device array), basepoint which is ManifoldArray. Main usecase is that Riemannian gradients are of type TangentArray.
    
    \item \texttt{rieoptax.core.rgrad:} Riemannian gradient operator.
\end{itemize}

\subsection{Geometries}

Geometry module contains manifolds equipped with different Riemannian metrics. Each Geometry contains Riemannian inner product \texttt{inp()}, induced norm \texttt{norm()}, Riemannian exponential \texttt{exp()}, logarithm maps \texttt{log()}, induced Riemannian distance \texttt{dist()}, parallel transport \texttt{pt()}, and transformation from the Euclidean gradient to Riemannian gradient \texttt{egrad\_to\_rgrad()}.

Manifolds include symmetric positive definite (SPD) matrices ${\rm SPD}(m) := \{ \mathbf X \in \mathbb R^{m \times m} : \mathbf X = \mathbf X^\top, \mathbf X \succ 0 \}$, hyperbolic space, Grassmann manifold $\mathcal{G}(m,r) := \{ [\mathbf X] : \mathbf X \in \mathbb R^{m \times r}, \mathbf X^\top \mathbf X = \mathbf I \}$ where $[\mathbf X] := \{ \mathbf {XO} : O \in O(r) \}$, $O(r)$ denotes the orthogonal group and hypersphere $\mathcal{S}(d) := \{ \mathbf x \in \mathbb R^d : \mathbf x^\top \mathbf x = 1 \}$. We use $T_x \mathcal M$ to represent the tangent space at $x$ and $\langle u,v \rangle_x$ to represent the Riemannian inner product. For more detailed treatment on these geometries, we refer to \cite{absil2009optimization,boumal2022intromanifolds,ungar2008gyrovector}.


% \AHcomment{(Shall we give some brief descriptions of the manifolds here? Because we need to benchmark in Section 3 and discuss size, etc.)} 


\begin{itemize}
    \item \texttt{rieoptax.geometry.spd.SPDAffineInvariant:} SPD matrices with the affine-invariant metric \cite{pennec2006riemannian}: SPD$(m)$ with $\langle \mathbf U, \mathbf V \rangle_{\mathbf X} = {\rm tr}( \mathbf X^{-1} \mathbf U \mathbf X^{-1} \mathbf V)$ for $\mathbf U, \mathbf V \in T_{\mathbf X} {\rm SPD}(m)$.
    
    \item \texttt{rieoptax.geometry.spd.SPDLogEuclidean:} SPD matrices with the Log-Euclidean metric \cite{arsigny2007geometric}: SPD$(m)$ with $\langle \mathbf U, \mathbf V \rangle_{\mathbf X} = {\rm tr} \big({\rm D}_{\mathbf U} {\rm logm}(\mathbf X) {\rm D}_{\mathbf V} {\rm logm}(\mathbf X) \big)$ where ${\rm D}_{\mathbf U} {\rm logm}(\mathbf X)$ is the directional derivative of matrix logarithm at $\mathbf X$ along $\mathbf U$.

    \item \texttt{rieoptax.geometry.hyperbolic.PoincareBall:} the Poincare-ball model of Hyperbolic space with Poincare metric \cite{ungar2008gyrovector}, i.e., $\mathbb D(d) := \{ \mathbf x \in \mathbb R^{d} : \mathbf x^\top \mathbf x < 1 \}$ with $\langle \mathbf u, \mathbf v \rangle_{\mathbf x} = 4\mathbf u^\top \mathbf v/(1 - \mathbf x^\top \mathbf x)^2$ for $\mathbf u, \mathbf v \in T_{\mathbf x} \mathbb D(d)$.
    
    \item \texttt{rieoptax.geometry.hyperbolic.LorentzHyperboloid:} the Lorentz Hyperboloid model of Hyperbolic space \cite{ungar2008gyrovector}, i.e., $\mathbb{H}(d) = \{ \mathbf{x} \in \mathbb{R}^{d} : \langle \mathbf x, \mathbf x \rangle_{\mathcal{L}}  = -1 \}$ with $\langle \mathbf u, \mathbf v \rangle_{\mathbf x} = \langle \mathbf u, \mathbf v \rangle_{\mathcal{L}}$ for $\mathbf u, \mathbf v \in T_{\mathbf x} \mathbb{H}(d)$, where $\langle \mathbf u, \mathbf v \rangle_{\mathcal{L}} := -u_0 v_0 + u_1 v_1 + \cdots u_{d-1} v_{d-1}$.
    
    \item \texttt{rieoptax.geometry.grassmann.GrassmannCanonicalMetric:} the Grassmann manifold with the canonical metric \cite{edelman1998geometry}, i.e., $\mathcal G(m,r)$ with $\langle  \mathbf{U}, \mathbf{V}\rangle_{\mathbf {X}}   = {\rm tr}\big( \mathbf{U}^{T} \mathbf{V} \big)$ for $\mathbf U, \mathbf V \in T_{\mathbf X} \mathcal G(m,r)$.
    
    \item  \texttt{rieoptax.geometry.hypersphere.HypersphereCanonicalMetric:} the hypersphere manifold which canonical metric \cite{absil2009optimization, boumal2022intromanifolds}, i.e., $\mathcal{S}(d)$ with $\langle \mathbf u, \mathbf v \rangle_{\textbf{x}} = \mathbf u^\top \mathbf v$ for $\mathbf u, \mathbf v \in T_{\mathbf x} \mathcal{S}(d)$.
\end{itemize}

\subsection{Optimizers}
Optimizers module contains Riemannian optimization algorithms. Design of optimizers follows Optax \cite{deepmind2020jax}, which implements every optimizer by chaining of few common transformations. Where every optimizer 
\begin{itemize}
    \item \texttt{riepotax.optimizers.first\_order.rsgd:} Riemannian stochastic gradient descent \cite{bonnabel2013stochastic}.

    \item \texttt{riepotax.optimizers.first\_order.rsvrg:}  Riemannian stochastic variance reduced gradient descent \cite{zhang2016riemannian}.
    
     \item \texttt{riepotax.optimizers.first\_order.rsrg:} Riemannian stochastic recursive gradient descent \cite{kasai2018riemannian}.
    
    \item \texttt{riepotax.optimizers.first\_order.rasa:} Riemannian adaptive stochastic gradient algorithm  \cite{kasai2019riemannian}.
    
    \item \texttt{riepotax.optimizers.zeroth\_order.zo\_rgd:} zeroth-order Riemannian gradient descent \cite{li2022stochastic}.
\end{itemize}

\subsection{Privacy mechanism}

Mechanism module contains differential private mechanisms on Riemannian manifolds.  

\begin{itemize}
    \item \texttt{rieoptax.mechanism.output\_perturbation.RieLaplaceMechanism:} the Riemannian Laplace mechanism \cite{reimherr2021differential} which is used for privatizing Fr\'echet mean computation. 
    
     \item \texttt{rieoptax.mechanism.output\_perturbation.LogEuclideanMechanism:} the Log-Euclidean mechanism \cite{utpala2022differentially} which is used for differentially private Fr\'echet mean on SPD matrices with log-Euclidean metric.
     
    \item \texttt{rieoptax.mechanism.gradient\_perturbation.DPRGDMechanism:} noise calibration for differentially private Riemannian gradient descent \cite{han2022differentially} based on moments accountant \cite{abadi2016deep} in the \texttt{autodp} library \cite{wang2019subsampled}. 
    
    \item \texttt{rieoptax.mechanism.gradient\_perturbation.DPRSGDMechanism:}  noise calibration for Differentially private Riemannian stochastic gradient descent \cite{han2022differentially} based on moments accountant \cite{abadi2016deep} in \texttt{autodp} library \cite{wang2019subsampled}. 
\end{itemize}




% \subsection{Example}

% We illustrate example  in 



\section{Benchmarking Rieoptax}
\label{sect:benchmark}
In this section, we benchmark the proposed Rieoptax against existing Riemannian optimization libraries in Python. These include Pytorch~\cite{paszke2019pytorch} based Mctorch~\cite{meghwanshi2018mctorch} and Geoopt~\cite{kochurov2020geoopt}, Tensorflow~\cite{smirnov2021tensorflow} based Tensorflow-Riemopt (Tf-Riemopt)~\cite{smirnov2021tensorflow}, Numpy~\cite{harris2020array} based Pymanopt \cite{JMLR:v17:16-177}, and Tensorflow based Geomstats \cite{miolane2020geomstats}. While Geomstats supports Numpy, Pytorch, and Tensorflow as backend, currently only the Tensorflow backend provides support for GPUs. 
% we observed error-free runs (on both GPU and CPU) only with Tensorflow backend. 
% \PJcomment{Sai - is this detail ok?}. 
% \AHcomment{Check now?}
Other non-Python based libraries include Manopt \cite{boumal2014manopt} in Matlab and Manopt.jl \cite{bergmann2022manopt} in Julia \cite{bezanson2017julia}.




%Geoopt \cite{kochurov2020geoopt}, Mctorch \cite{meghwanshi2018mctorch} are based on Pytorch \cite{paszke2019pytorch} and Tensorflow-Riemopt (Tf-Riemopt) \cite{smirnov2021tensorflow} based on tensorflow \cite{smirnov2021tensorflow}. Pymanopt \cite{JMLR:v17:16-177} is based on Numpy \cite{harris2020array}, and Geomstats \cite{miolane2020geomstats} \AHcomment{(Unfinished here)}. Some other frameworks in other languages include  Manopt \cite{boumal2014manopt} in Matlab, Manopt.jl \cite{bergmann2022manopt} in Julia \cite{bezanson2017julia}. 
We benchmark the Riemannian exponential (Exp) and logarithm (Log) maps with the proposed Rieoptax against the aforementioned Python libraries whenever available with \texttt{64bitfloat} precision. For CPU benchmarking, we use the AMD EPYC 7B1 processor with 2 cores and 16{GB} RAM. For GPU benchmarking, we use {CUDA} version $11.0$ on 16{GB} Tesla {P100}.
%Geoopt \cite{kochurov2020geoopt}, Mctorch \cite{meghwanshi2018mctorch} are based on Pytorch \cite{paszke2019pytorch} and Tensorflow-Riemopt (Tf-Riemopt) \cite{smirnov2021tensorflow} based on tensorflow \cite{smirnov2021tensorflow}. Pymanopt \cite{JMLR:v17:16-177} is based on Numpy \cite{harris2020array}, and Geomstats \cite{miolane2020geomstats} \AHcomment{(Unfinished here)}. Some other frameworks in other languages include  Manopt \cite{boumal2014manopt} in Matlab, Manopt.jl \cite{bergmann2022manopt} in Julia \cite{bezanson2017julia}. 
% We benchmark the Riemannian exponential (Exp) and logarithm (Log) maps with the proposed Rieoptax against the aforementioned Python libraries whenever available. For GPU benchmarking, we use {CUDA} version $11.4$ on 16{GB} Tesla {P100}.



% \cite{bu2021fast} proposed algorithmic solution for approximate computation of per-example gradient norms based on celebrated Johnson-Lindenstrauss lemma \cite{article,dasgupta2003elementary}.  There is architecture specific way of \cite{goodfellow2015efficient, }. Contrary to this, \cite{subramani2021enabling} showed how to exploit compiler optimization techniques like  Just-in-Time compilation (\textsf{JIT}), Vectorization and Static graph optimization significantly  speedup the Differentially private stochastic gradient descent \textsf{DP-SGD}. This approach is readily applicable to applicable to Riemannian case. 


% \begin{figure} \centering
%     \begin{subfigure}[b]{60mm}
%         \includegraphics[width=60mm]{plots/cpu/Grassmann_cpu_exp.pdf}
%         \label{fig:a}
%     \end{subfigure} %

%     \begin{subfigure}[b]{60mm}    
%         \includegraphics[width=60mm]{plots/cpu/Grassmann_cpu_log.pdf}
%         \label{fig:b}    
%     \end{subfigure} 
%     \caption{my caption}
% \end{figure}


\begin{figure}[t]
\centering     %%% not \center
\subfigure[Hypersphere Exp]{\label{fig:HypExp1}\includegraphics[width=35mm]{plots/cpu/hypersphere_cpu_exp.pdf}}
\subfigure[Lorentz Exp]{\label{fig:LorExp1}\includegraphics[width=35mm]{plots/cpu/LH_cpu_exp.pdf}}
\subfigure[Grassmann Exp]{\label{fig:GrassExp1}\includegraphics[width=35mm]{plots/cpu/Grassmann_cpu_exp.pdf}}
\subfigure[SPD Exp]{\label{fig:LorLog1}\includegraphics[width=35mm]{plots/cpu/SPD_cpu_exp.pdf}}

\subfigure[Hypersphere Log]{\label{fig:HypLog2}\includegraphics[width=35mm]{plots/cpu/hypersphere_cpu_log.pdf}}
\subfigure[Lorentz Log]{\label{fig:LorExp2}\includegraphics[width=35mm]{plots/cpu/LH_cpu_log.pdf}}
\subfigure[Grassmann Log]{\label{fig:GrassLog2}\includegraphics[width=35mm]{plots/cpu/Grassmann_cpu_log.pdf}}
\subfigure[SPD  Log]{\label{fig:LorLog2}\includegraphics[width=35mm]{plots/cpu/SPD_cpu_log.pdf}}
\caption{Benchmarking of geometric primitives on CPU.}\label{fig:CPUresults}
\end{figure}





\begin{figure}[t]
\centering     %%% not \center
\subfigure[Hypersphere Exp]{\label{fig:HypExp3}\includegraphics[width=35mm]{plots/gpu/hypersphere_gpu_exp.pdf}}
\subfigure[Lorentz Exp]{\label{fig:LorExp3}\includegraphics[width=35mm]{plots/gpu/LH_gpu_exp.pdf}}
\subfigure[Grassmann Exp]{\label{fig:GrassExp3}\includegraphics[width=35mm]{plots/gpu/Grassmann_gpu_exp.pdf}}
\subfigure[SPD Exp]{\label{fig:LorLog3}\includegraphics[width=35mm]{plots/gpu/SPD_gpu_exp.pdf}}

\subfigure[Hypersphere Log]{\label{fig:HypExp}\includegraphics[width=35mm]{plots/gpu/hypersphere_gpu_log.pdf}}
\subfigure[Lorentz Log]{\label{fig:LorExp}\includegraphics[width=35mm]{plots/gpu/LH_gpu_log.pdf}}
\subfigure[Grassmann Log]{\label{fig:GrassExp}\includegraphics[width=36mm]{plots/gpu/Grassmann_gpu_log.pdf}}
\subfigure[SPD Log]{\label{fig:LorLog}\includegraphics[width=35mm]{plots/gpu/SPD_gpu_log.pdf}}

\caption{Benchmarking of geometric primitives on GPU.}\label{fig:GPUresults}
\end{figure}



\begin{itemize}
    \item  \textbf{Hypersphere:}  hypersphere $\mathcal{S}(d)$ is supported in Geoopt, Tf-Riemopt, Geomstats, McTorch, and Pyamanopt. McTorch does not support the Exp and Log maps. On GPU, Geomstats raises an error. We benchmark all expect McTorch and Geomstats for dimensions $ d \in \{50, 100,  500, 1\,000, 5\,000, 10\,000, 25\,000, 50\,000 \}$. 

    \item \textbf{Loretnz hyperboloid model:} the Loretnz hyperboloid model $\mathbb{H}(d)$ is supported in Geoopt, Tf-Riemopt, Geomstats, and Mctorch. While the Exp map is available in Mctorch, it does not implement the Log map. We benchmark for dimensions $d \in \{50, 100,  500, 1\,000, 5\,000,$ $10\,000, 25\,000, 50\,000\}$.  

    
    \item \textbf{Grassmann:} Grassmann manifold $\mathcal{G}(m,r)$ is supported in Tf-Riemopt, Pymanopt, McTorch, and Geomstats. McTorch does not support the Exp and Log maps. 
    Geomstats represents Grassmann elements in projector matrices form $\mathbf X \mathbf X^\top \in \mathbb R^{m \times m}$ instead of  $\mathbf X \in \mathbb R^{m \times r}$, which is prohibitively expensive. We, therefore, exclude these three libraries from benchmarking. We benchmark for matrix sizes $(m,r) \in \{ (100,10) ,(500, 10), \allowbreak (750, 10), (1\,000, 10), (2\,000,10), (5\,000, 10) \}$.
    
    \item \textbf{SPD with affine-invariant metric:} SPD manifold ${\rm SPD}(m)$ with the affine-invariant metric is supported in Geoopt, Tf-Riemopt, Geomstats, and McTorch. McTorch, however, does not support the Exp and Log maps. We benchmark all except McTorch for matrix sizes
    $m \in \{10, 50, 75, 100,  150,  200 \}$.
\end{itemize}
Figures~\ref{fig:CPUresults} and~\ref{fig:GPUresults} present the timing results with CPU- and GPU-based computations, respectively. Overall, we observe that Rieoptax offers significant time improvements, especially on GPUs. For the SPDAffineInvariant case, Rieoptax is slightly slower than Geoopt because \texttt{eigh} which provides eigen decomposition is slightly slower in JAX compared to Pytorch. 
%Rieoptax is faster in all cases except for the one on SPD manifold with affine invariant metric. In this case, Geoopt is slightly faster. 
Given that JAX is a relatively new framework, we believe it would be faster even in this case in the near future. 


\begin{listing}
\begin{mdframed}
\begin{Verbatim}[commandchars=\\\{\}]
\PYG{k+kn}{from} \PYG{n+nn}{jax} \PYG{k+kn}{import} \PYG{n}{jit}\PYG{p}{,} \PYG{n}{vmap}
\PYG{k+kn}{from} \PYG{n+nn}{jax.numpy.linalg} \PYG{k+kn}{import} \PYG{n}{norm}
\PYG{k+kn}{from} \PYG{n+nn}{rieoptax.core} \PYG{k+kn}{import} \PYG{n}{rgrad}\PYG{p}{,} \PYG{n}{ManifoldArray}
\PYG{k+kn}{from} \PYG{n+nn}{rieoptax.geometry.grassmann} \PYG{k+kn}{import} \PYG{n}{GrassmannCanonical}
\PYG{k+kn}{from} \PYG{n+nn}{rieoptax.optimizer.first\PYGZus{}order} \PYG{k+kn}{import} \PYG{n}{rsgd}\PYG{p}{,} \PYG{n}{dp\PYGZus{}rsgd}
\PYG{k+kn}{from} \PYG{n+nn}{rieoptax.mechanism.gradient\PYGZus{}perturbation} \PYG{k+kn}{import} \PYG{n}{DP\PYGZus{}RGD\PYGZus{}Mechanism}
\PYG{k+kn}{from} \PYG{n+nn}{rieoptax.optimizer.update} \PYG{k+kn}{import} \PYG{n}{apply\PYGZus{}updates}

\PYG{k}{def} \PYG{n+nf}{fit}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{data}\PYG{p}{,} \PYG{n}{optimizer}\PYG{p}{,} \PYG{n}{epochs}\PYG{p}{,} \PYG{n}{private}\PYG{o}{=}\PYG{k+kc}{False}\PYG{p}{):}

    \PYG{k}{def} \PYG{n+nf}{step}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state}\PYG{p}{,} \PYG{n}{data}\PYG{p}{):}
        \PYG{k}{def} \PYG{n+nf}{cost}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{data}\PYG{p}{):}
            \PYG{k}{def} \PYG{n+nf}{\PYGZus{}cost}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{data}\PYG{p}{):}
                \PYG{k}{return} \PYG{n}{norm}\PYG{p}{(}\PYG{n}{data}\PYG{o}{\PYGZhy{}}\PYG{n}{params}\PYG{o}{.}\PYG{n}{value}\PYG{o}{@}\PYG{p}{(}\PYG{n}{params}\PYG{o}{.}\PYG{n}{value}\PYG{o}{.}\PYG{n}{T} \PYG{o}{@} \PYG{n}{data}\PYG{p}{))}\PYG{o}{**}\PYG{l+m+mi}{2}
            \PYG{k}{return} \PYG{n}{vmap}\PYG{p}{(}\PYG{n}{\PYGZus{}cost}\PYG{p}{,} \PYG{n}{in\PYGZus{}axes}\PYG{o}{=}\PYG{p}{(}\PYG{k+kc}{None}\PYG{p}{,}\PYG{l+m+mi}{0}\PYG{p}{))(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{data}\PYG{p}{)}\PYG{o}{.}\PYG{n}{mean}\PYG{p}{()}

        \PYG{n}{rgrad\PYGZus{}fn} \PYG{o}{=} \PYG{n}{rgrad}\PYG{p}{(}\PYG{n}{cost}\PYG{p}{)}
        \PYG{k}{if} \PYG{n}{private}\PYG{p}{:}
            \PYG{n}{data} \PYG{o}{=} \PYG{n}{data}\PYG{p}{[:,} \PYG{k+kc}{None}\PYG{p}{]}
            \PYG{n}{rgrad\PYGZus{}fn} \PYG{o}{=} \PYG{n}{vmap}\PYG{p}{(}\PYG{n}{rgrad\PYGZus{}fn}\PYG{p}{,} \PYG{n}{in\PYGZus{}axes}\PYG{o}{=}\PYG{p}{(}\PYG{k+kc}{None}\PYG{p}{,} \PYG{l+m+mi}{0}\PYG{p}{))}\PYG{c+c1}{\PYGZsh{}per\PYGZhy{}example gradient}
        \PYG{n}{rgrads} \PYG{o}{=} \PYG{n}{rgrad\PYGZus{}fn}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{data}\PYG{p}{)}\PYG{c+c1}{\PYGZsh{}calculates Riemannian gradients}
        \PYG{n}{updates}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state} \PYG{o}{=} \PYG{n}{optimizer}\PYG{o}{.}\PYG{n}{update}\PYG{p}{(}\PYG{n}{rgrads}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state}\PYG{p}{,} \PYG{n}{params}\PYG{p}{)}
        \PYG{n}{params} \PYG{o}{=} \PYG{n}{apply\PYGZus{}updates}\PYG{p}{(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{updates}\PYG{p}{)}\PYG{c+c1}{\PYGZsh{}update using Riemannian Exp}
        \PYG{k}{return} \PYG{n}{params}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state}\PYG{p}{,} \PYG{n}{loss\PYGZus{}value}

    \PYG{n}{opt\PYGZus{}state} \PYG{o}{=} \PYG{n}{optimizer}\PYG{o}{.}\PYG{n}{init}\PYG{p}{(}\PYG{n}{params}\PYG{p}{)}
    \PYG{k}{for} \PYG{n}{i} \PYG{o+ow}{in} \PYG{n+nb}{range}\PYG{p}{(}\PYG{n}{epochs}\PYG{p}{):}
        \PYG{n}{params}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state}\PYG{p}{,} \PYG{n}{loss\PYGZus{}value} \PYG{o}{=} \PYG{n}{jit}\PYG{p}{(}\PYG{n}{step}\PYG{p}{)(}\PYG{n}{params}\PYG{p}{,} \PYG{n}{opt\PYGZus{}state}\PYG{p}{,} \PYG{n}{data}\PYG{p}{)}

\PYG{c+c1}{\PYGZsh{}initialization}
\PYG{n}{U\PYGZus{}init} \PYG{o}{=} \PYG{n}{ManifoldArray}\PYG{p}{(}\PYG{n}{value}\PYG{o}{=}\PYG{n}{init}\PYG{p}{,} \PYG{n}{manifold}\PYG{o}{=}\PYG{n}{GrassmannCanonical}\PYG{p}{())}

\PYG{c+c1}{\PYGZsh{} non private PCA}
\PYG{n}{lr}\PYG{p}{,} \PYG{n}{epochs} \PYG{o}{=} \PYG{p}{(}\PYG{l+m+mf}{3e\PYGZhy{}3}\PYG{p}{,} \PYG{l+m+mi}{400}\PYG{p}{)}
\PYG{n}{optimizer} \PYG{o}{=} \PYG{n}{rsgd}\PYG{p}{(}\PYG{n}{lr}\PYG{p}{)}
\PYG{n}{non\PYGZus{}private\PYGZus{}U} \PYG{o}{=} \PYG{n}{fit}\PYG{p}{(}\PYG{n}{U\PYGZus{}init}\PYG{p}{,} \PYG{n}{Z}\PYG{p}{,} \PYG{n}{optimizer}\PYG{p}{,} \PYG{n}{epochs}\PYG{p}{)}

\PYG{c+c1}{\PYGZsh{}(eps, delta) differentially private PCA}
\PYG{n}{eps}\PYG{p}{,} \PYG{n}{delta}\PYG{p}{,} \PYG{n}{clip\PYGZus{}norm}\PYG{p}{,} \PYG{n}{epochs} \PYG{o}{=} \PYG{p}{(}\PYG{l+m+mf}{1.0}\PYG{p}{,} \PYG{l+m+mf}{1e\PYGZhy{}6}\PYG{p}{,} \PYG{l+m+mf}{0.1}\PYG{p}{,} \PYG{l+m+mi}{200}\PYG{p}{)}
\PYG{n}{sigma} \PYG{o}{=} \PYG{n}{DP\PYGZus{}RGD\PYGZus{}Mechanism}\PYG{p}{(}\PYG{n}{eps}\PYG{p}{,} \PYG{n}{delta}\PYG{p}{,} \PYG{n}{clip\PYGZus{}norm}\PYG{p}{,} \PYG{n}{n}\PYG{p}{)}
\PYG{n}{private\PYGZus{}optimizer} \PYG{o}{=} \PYG{n}{dp\PYGZus{}rsgd}\PYG{p}{(}\PYG{n}{lr}\PYG{p}{,} \PYG{n}{sigma}\PYG{p}{,} \PYG{n}{clip\PYGZus{}norm}\PYG{p}{)}
\PYG{n}{private\PYGZus{}U} \PYG{o}{=} \PYG{n}{fit}\PYG{p}{(}\PYG{n}{U\PYGZus{}init}\PYG{p}{,} \PYG{n}{Z}\PYG{p}{,} \PYG{n}{optimizer}\PYG{p}{,} \PYG{n}{epochs}\PYG{p}{,} \PYG{n}{private}\PYG{o}{=}\PYG{k+kc}{True}\PYG{p}{)}
\end{Verbatim}
\end{mdframed}
\caption{Rieoptax code for the principal component analysis (PCA) problem on the Grassmann manifold, where initialization (\texttt{init}) and sample matrix (\texttt{Z}) are user inputs.}
\label{list:code}
\end{listing}

% \begin{listing}
% \begin{mdframed}
% \begin{lstlisting}[language=Python]
% from jax import jit, vmap
% from jax.numpy.linalg import norm 
% from rieoptax.core import rgrad, ManifoldArray
% from rieoptax.geometry.grassmann import GrassmannCanonical
% from rieoptax.optimizer.first_order import rsgd, dp_rsgd
% from rieoptax.mechanism.gradient_perturbation import DP_RGD_Mechanism
% from rieoptax.optimizer.update import apply_updates

% def fit(params, data, optimizer, epochs, private=False):

%     def step(params, opt_state, data):
%         def cost(params, data):
%             def _cost(params, data):
%                 return norm(data-params.value@(params.value.T @ data))**2
%             return vmap(_cost, in_axes=(None,0))(params, data).mean()
            
%         rgrad_fn = rgrad(cost)
%         if private:
%             data = data[:, None]
%             rgrad_fn = vmap(rgrad_fn, in_axes=(None, 0))#per-example gradient
%         rgrads = rgrad_fn(params, data)#calculates Riemannian gradients 
%         updates, opt_state = optimizer.update(rgrads, opt_state, params)
%         params = apply_updates(params, updates)#update using Riemannian Exp
%         return params, opt_state, loss_value
    
%     opt_state = optimizer.init(params)
%     for i in range(epochs):
%         params, opt_state, loss_value = jit(step)(params, opt_state, data)

% #initialization
% U_init = ManifoldArray(value=init, manifold=GrassmannCanonical())
        
% # non private PCA
% lr, epochs = (3e-3, 400)
% optimizer = rsgd(lr)
% non_private_U = fit(U_init, Z, optimizer, epochs)

% #(eps, delta) differentially private PCA
% eps, delta, clip_norm, epochs = (1.0, 1e-6, 0.1, 200)
% sigma = DP_RGD_Mechanism(eps, delta, clip_norm, n)
% private_optimizer = dp_rsgd(lr, sigma, clip_norm) 
% private_U = fit(U_init, Z, optimizer, epochs, private=True)
% \end{lstlisting}

% \end{mdframed}

% \end{listing}




\begin{figure}[h!]
\centering     %%% not \center
\subfigure[Non-private PCA.]{\label{fig:NonPrivatePCA}\includegraphics[width=50mm]{plots/NonPrivatePCA.pdf}}
\subfigure[$(0.1, 10^{-6})$-private PCA.]{\label{fig:PrivatePCA}\includegraphics[width=50mm]{plots/PrivatePCA.pdf}}
\caption{Timing of Rieoptax for PCA on the TinyImagetNet dataset as optimization on Grassmann manifold $\mathcal{G}(12\,288, 5)$ on both CPU and GPU. The GPU implementation achieves a significant
% $85\times$ and $130\times$ 
speedup than CPU on both non-private and private PCA problems. 
% \STcomment{not true right?!} 
% Also, we see that the time difference between non-private and private implementations is negligible on GPU.
}
\end{figure}





\section{An example on PCA}


In this section, we consider the problem of principal components analysis (PCA) by viewing it as an optimization problem on the Grassmann manifold \cite{boumal2022intromanifolds,absil2009optimization}, i.e.,
\begin{align}\label{eq:pca}
    \min_{\textbf{U} \in \mathcal{G}(m, r)} \frac{1}{n} \sum_{i=1}^{n} \norm{\textbf{z}_{i} - \textbf{U}\textbf{U}^T \textbf{z}_i}_{2}^2,
\end{align}
where $\textbf{z}_i \in \mathbb{R}^n$ denote the data points. The Rieoptax implementation for solving the problem (\ref{eq:pca}) is shown in Listing \ref{list:code}.

We provide timing of Rieoptax on TinyImageNet \cite{le2015tiny}  which has a training set of $10^{5}$ images in dimensions of $3 \times 64 \times 64$ on both CPU and GPU. We take $5\,000$ images and vectorize each image to produce a sample matrix of size $(n, d) = (5\,000, 12\,288)$. We compute the top $r = 5$ principal components, which leads to an optimization problem on $\mathcal{G}(12\,288, 5)$. 

For non-private PCA, we run the full Riemannian gradient descent method for 400 epochs. For private PCA, we run the differentially private Riemannian gradient descent method \cite{han2022differentially} for $200$ epochs with a privacy configuration of $\epsilon = 0.1, \delta = 10^{-6}$ and gradient clipping parameter of $0.1$. For both the private and non-private algorithms, we choose the same initialization and a learning rate of $3\times10^{-3}$. Figures~\ref{fig:NonPrivatePCA} and \ref{fig:PrivatePCA} show excess risk against runtime (in seconds) for non-private and private PCA, respectively. 












\section{Conclusion and future roadmap}
In this work, we present a Python library for (privacy-supported) Riemannian optimization, Rieoptax, and illustrate its efficacy on both CPU and GPU architectures. Our roadmap includes adding support for more manifold geometries, optimization algorithms, and a collection of example codes showcasing the usage of Rieoptax in various applications, especially with differential privacy.

%Preliminary work that demonstrates that JAX. We plan to add 


